Exploring the Design Space of Longitudinal Censorship Measurement Platforms

Despite the high perceived value and increasing severity of online information controls, a data-driven understanding of the phenomenon has remained elusive. In this paper, we consider two design points in the space of Internet censorship measurement with particular emphasis on how they address the challenges of locating vantage points, choosing content to test, and analyzing results. We discuss the trade offs of decisions made by each platform and show how the resulting data provides complementary views of global censorship. Finally, we discuss lessons learned and open challenges discovered through our experiences.

==> Makefile <==
###########################################################
#
# Makefile for LaTeX docs
#

TEX = main
FIGS = 
PSFIGS = $(FIGS:.pdf=.ps)

all: pdf
ps:  $(TEX).ps
pdf: $(TEX).pdf
dvi: $(TEX).dvi

clean:
	$(RM) *.out *.aux *.log *.bbl *.blg *~ \#*\# *.toc *.idx *.eps dummy
	$(RM) $(patsubst %.tex, %.ps, $(wildcard *.tex))
	$(RM) $(patsubst %.tex, %.dvi, $(wildcard *.tex))
	$(RM) $(patsubst %.tex, %.pdf, $(wildcard *.tex))

# only need -Ppdf if using CM fonts

main.pdf: *.tex main.bib Makefile
	pdflatex main.tex
	bibtex main
	pdflatex main.tex
	pdflatex main.tex

# This is for a tool of mine that monitors files for changes via
# inotify and then executes actions. --cpk
notif:
	notif -vv *.tex *.bib make

